ARCADE: Scalable Demonstration Collection and Generation via Augmented Reality for Imitation Learning

Robot Imitation Learning (IL) is a crucial technique in robot learning, where agents learn by mimicking human demonstrations. However, IL encounters scalability challenges stemming from both non-user-friendly demonstration collection methods and the extensive time required to amass a sufficient number of demonstrations for effective training. In response, we introduce the Augmented Reality for Collection and generAtion of DEmonstrations (ARCADE) framework, designed to scale up demonstration collection for robot manipulation tasks. Our framework combines two key capabilities: 1) it leverages AR to make demonstration collection as simple as users performing daily tasks using their hands, and 2) it enables the automatic generation of additional synthetic demonstrations from a single human-derived demonstration, significantly reducing user effort and time. We assess ARCADE's performance on a real Fetch robot across three robotics tasks: 3-Waypoints-Reach, Push, and Pick-And-Place. Using our framework, we were able to rapidly train a policy using vanilla Behavioral Cloning (BC), a classic IL algorithm, which excelled across these three tasks. We also deploy ARCADE on a real household task, Pouring-Water, achieving an 80% success rate.

==> 03_preliminaries.tex <==
\section{Preliminaries}
In this section, we introduce the three building blocks of ARCADE: Markov Decision Process, Behavioral Cloning, and Dynamic Time Warping.

% % MDP
\subsection{Markov Decision Process}
We consider a Markov Decision Process (MDP)~\cite{white1993survey}, denoted as $\mathcal{M}=\langle\mathcal{S}, \mathcal{A}, R, T, \gamma, \rho_0\rangle$. Here, $\mathcal{S}$ is the state space, and $\mathcal{A}$ denotes the action space. The function $R : \mathcal{S}\rightarrow \mathbb{R}$ is the reward given a state. The deterministic transition function $T : \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S}$ determines the subsequent state $s'$ upon applying action $a$ in state $s$. $\gamma \in (0, 1)$ denotes the temporal discount factor. $\rho_0 : \mathcal{S} \rightarrow \mathbb{R}$ represents the initial state probability distribution. The agent behavior is defined by a stochastic policy $\pi : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$, which is a mapping from states to probabilities over actions. In this work, we use an MDP without an explicitly defined reward function, i.e., $M \backslash R$. 

% A trajectory $\tau = (s_0, a_0, \cdots, s_t, a_t, \cdots)$ is generated by executing policy $\pi$ within this environment, following $s_0\sim \rho_0, a_t\sim\pi(s_t), s_{t+1}=T(s_t,a_t)\ \forall t\geq 0$. The expected discounted return of a policy $\pi$ is given by $J(\pi) = \mathbb{E}{\tau \sim \pi}\left[\sum^\infty{t=0}\gamma^t R(s_t)\right]$. The goal in Reinforcement Learning (RL) is to identify the optimal policy, $\pi^*$, which maximizes $J(\pi)$.

% $\mathcal{M}=\langle\mathcal{S}, \mathcal{A}, R, T, \gamma, \rho_0\rangle$. $\mathcal{S}$ and $\mathcal{A}$ denote the state and action space, respectively. $R: \mathcal{S}\rightarrow \mathbb{R}$ is the reward of a given state. $T : \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S}$ is a deterministic transition function that gives the next state, $s'$, for applying the action, $a$, in state, $s$. $\gamma \in (0, 1)$ is the temporal discount factor. $\rho_0 : \mathcal{S} \rightarrow \mathbb{R}$ denotes the initial state probability distribution. A stochastic policy $\pi : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ is a mapping from states to probabilities over actions. A trajectory, $\tau = (s_0, a_0, \cdots, s_t, a_t, \cdots)$, is generated by executing the policy within the environment: $s_0\sim \rho_0, a_t\sim\pi(s_t), s_{t+1}=T(s_t,a_t)\ \forall t\geq 0$. The expected discounted return of a policy, $\pi$, is calculated by $J(\pi) = \mathbb{E}_{\tau \sim \pi}\left[\sum^\infty_{t=0}\gamma^t R(s_t)\right]$. The objective for RL is to find the optimal policy, $\pi^* = \argmax_{\pi} J(\pi)$.



% BC
\subsection{Behavioral Cloning}
Behavioral cloning (BC)~\cite{pomerleau1988alvinn}, a classic method in IL, involves training a policy to mimic demonstrations collected by an oracle (e.g., an end-user). We denote demonstrations as $\Xi = \{\tau_i\}_{i=1}^M$, where each demonstration is a list of state-action pairs, $\mathcal{\tau} = \{(s_i, a_i)\}_{i=1}^{N}$. BC aims to learn a policy $\pi_{\theta}$, parameterized by $\theta$, from given demonstrations $\Xi$. The objective is to solve the optimization problem shown in Equation~\ref{eq:obj_bc}.
\begin{equation}
\label{eq:obj_bc}
    \hat{\pi} = \arg\min_{\theta}\sum_{\tau\in\mathcal{D}}\sum_{(s, a)\in\tau}\mathcal{L}(\pi_{\theta}(s), a),
\end{equation}
where $\hat{\pi}$ is the objective policy. $\mathcal{L}$ is the cost function.






% DTW
\subsection{Dynamic Time Warping}
\label{subsec:dtw}
Dynamic Time Warping (DTW)~\cite{muller2007dynamic} is an algorithm used for quantifying the similarity between two temporal sequences, $ \mathcal{X} \coloneqq \{x_i\}_{i=1}^{U} $ and $ \mathcal{Y} \coloneqq \{y_j\}_{j=1}^{V} $, which may differ in timing or speed. It involves computing a distance matrix $ \mathcal{D} $, where each element $ \mathcal{D}[i, j] $ represents the distance between $ x_i $ and $ y_j $. The goal is to determine the path, $\mathcal{P}$, within this matrix that minimizes the total distance, thereby optimizing the alignment of the sequences. Equation~\ref{eq:dtw} details the DTW similarity of the two sequences.
\begin{equation}
\label{eq:dtw}
    \mathcal{DTW}(\mathcal{X}, \mathcal{Y}) = \min \sqrt{\sum_{(i, j) \in \mathcal{P}} d(x_i, y_j)^2},
\end{equation}
where $ d(x_i, y_j) $ is the distance between elements. 





